On Greedily Packing Anchored Rectangles

Consider a set P of points in the unit square U, one of them being the origin. For each point p in P you may draw a rectangle in U with its lower-left corner in p. What is the maximum area such rectangles can cover without overlapping each other? Freedman [1969] posed this problem in 1969, asking whether one can always cover at least 50% of U. Over 40 years later, Dumitrescu and T\'oth [2011] achieved the first constant coverage of 9.1%; since then, no significant progress was made. While 9.1% might seem low, the authors could not find any instance where their algorithm covers less than 50%, nourishing the hope to eventually prove a 50% bound. While we indeed significantly raise the algorithm's coverage to 39%, we extinguish the hope of reaching 50% by giving points for which the coverage is below 43.3%. Our analysis studies the algorithm's average and worst-case density of so-called tiles, which represent the area where a given point can freely choose its maximum-area rectangle. Our approachis comparatively general and may potentially help in analyzing related algorithms.

==> 80-conclusion.tex <==
\section{Conclusion}
\christoph{remove or write conclusion}
Some ideas on improving the ratio further:
\begin{itemize}
    \item {
        Cut crowns from below or left. This will decrease the crown area, but also decrease the total area the crowns will fit into. This is basically the same as the $\lambda$-cutting of Dumitrescu's and Tóth's trapezoids.
    }
    \item {
        The upper bound does not only hold when we already built all the tiles, but it also
        holds at each step in between. If we have tiles of total area $T$ already built, and their crowns
        fit into an area of at most $C$, we can provide a lower bound on the fraction they cover.
        
        Consider all points in $P$ that lie on the pareto front of $(1,0)$ (to the top left of $(1,0)$).
        If this front is not too close to the point
        $(1,0)$ itself, then the crowns cannot reach certain lower parts of the $U$ (and the triangle attached at the bottom of $U$). The same would work if we flip the $x$/$y$-axis (pareto front around $(0,1)$). However, if the pareto fronts are very close to these points on both sides, then...?
    }
    \item {
        Interestingly, in the upper bound example,
        all tiles except the $(0,0)$-tile have roughly the
        same total size as their crowns. Using \Cref{thm:low_crown_size_fifty_percent}, it seems that this is the best upper bound derivable when
        the $(0,0)$-tile is fixed.
    }
    \item {
        We believe that a similar charging scheme might extend to other (anchored) rectangle packing problems.
    }
    \item {
        Our proof in principle generalizes to other container shapes.
        You just have to put a lower bound on the total tile areas and
        an upper bound on the total crown area (which is easy to determine once you know the former, since you just extend triangles to the lower left).
    }
    \item {
        where does the discontinuity in the lower bound come from?
    }
    \item {
        where do we lose percent points something in our lower bound calculation?
    }
    \item {
        ideas for improving the algorithm?
    }
\end{itemize}
